SeaKR: Self-aware Knowledge Retrieval for Adaptive Retrieval Augmented Generation

This paper introduces Self-aware Knowledge Retrieval (SeaKR), a novel adaptive RAG model that extracts self-aware uncertainty of LLMs from their internal states. SeaKR activates retrieval when the LLMs present high self-aware uncertainty for generation. To effectively integrate retrieved knowledge snippets, SeaKR re-ranks them based on LLM's self-aware uncertainty to preserve the snippet that reduces their uncertainty to the utmost. To facilitate solving complex tasks that require multiple retrievals, SeaKR utilizes their self-aware uncertainty to choose among different reasoning strategies. Our experiments on both complex and simple Question Answering datasets show that SeaKR outperforms existing adaptive RAG methods. We release our code at https://github.com/THU-KEG/SeaKR.

==> table/3-uncertainty.tex <==
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrrrrrr}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{NQ} & \multicolumn{2}{c}{2Wiki} & \multicolumn{2}{c}{HPQA} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
& 
\multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} \\
\midrule
Perplexity & $24.2$ & $35.1$& $00.0$& $00.0$& $00.0$& $00.0$\\
Energy & $23.8$  & $32.9$ & \\
LN Entropy & $27.8$ & $37.5$ &\\
\midrule
Eigen Score & $\mathbf{29.0}$ & $\mathbf{38.9}$ \\
\bottomrule
\end{tabular}
}
\caption{Comparison of other uncertainty measurement on reranking documents.}
\label{tab:uncertainty-reranking}
\end{table}

% \model & -&-&0.356&0.4767&0.258&0.3003 \\ %llama3-8b-instruct


% \model & -&-&0.356&0.4767&0.258&0.3003 \\ %llama3-8b-instruct

==> table/4-synthesize-results.tex <==
\begin{table}[]
\centering
\scalebox{0.95}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrrrrrrrrrr}
\toprule
\multirow{2}{*}{Model} &  \multicolumn{2}{c}{2Wiki} & \multicolumn{2}{c}{HPQA}  \\
\cmidrule(r){2-3} \cmidrule(r){4-5} & 
\multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \\
\midrule
Final Step & \\
CoT Reader & \\
Adaptive & \\
\bottomrule
\end{tabular}
}
\caption{Comparison of different final answer aggregation strategies in multihop reasoning. "Final Step" strategy extracts the answer directly from the final step generated. CoT Reader uses a posthoc CoT Reader that takes all retrieved passages and the query, generating new CoT steps and an answer. The "Adaptive" strategy adaptively chooses either method based on their average eigen score across different steps.}
\label{tab:synthesis}
\end{table}

% \model & -&-&0.356&0.4767&0.258&0.3003 \\ %llama3-8b-instruct
